MACH: Multi-Agent Coordination for RSU-centric Handovers

This paper introduces MACH, a novel approach for optimizing task handover in vehicular computing scenarios. To ensure fast and latency-aware placement of tasks, the decision-making -- where and when should tasks be offloaded -- is carried out decentralized at the Road Side Units (RSUs) who also execute the tasks. By shifting control to the network edge, MACH moves away from the traditional centralized or vehicle-based handover method. Still, it focuses on contextual factors, such as the current RSU load and vehicle trajectories. Thus, MACH improves the overall Quality of Service (QoS) while fairly balancing computational loads between RSUs. To evaluate the effectiveness of our approach, we develop a robust simulation environment composed of real-world traffic data, dynamic network conditions, and different infrastructure capacities. For scenarios that demand low latency and high reliability, our experimental results demonstrate how MACH significantly improves the adaptability and efficiency of vehicular computations. By decentralizing control to the network edge, MACH effectively reduces communication overhead and optimizes resource utilization, offering a robust framework for task handover management.

==> sections/2_preliminaries.tex <==
\chapter{Preliminaries} \label{sec:2_preliminaries}

This chapter provides essential background for the thesis. 
We begin with an overview of \gls{ec} (Section~\ref{sec:2_prelim:edge_computing}), focusing on \gls{mec} (Section~\ref{sec:2_prelim:ec:mec}) and \gls{vec} (Section~\ref{sec:2_prelim:ec:vec}). 
These sections will cover the fundamental concepts, technologies, and \gls{ec} applications, emphasizing mobile and vehicular contexts. 
For a concise comparison of these paradigms, refer to Table~\ref{tab:2_prelim:ec_mec_vec_comparison} at the end of Section~\ref{sec:2_prelim:ec:vec}.
Finally, we discuss \glspl{mas} (Section~\ref{sec:2_prelim:mas}), including their architecture, applications, and associated challenges. 
%We then examine communication patterns in distributed systems (Section~\ref{sec:2_prelim:comm_patterns}), highlighting both general and \gls{mas}-specific patterns. 
% Finally, we explore the integration of \glspl{mas} and \gls{vec} (Section~\ref{sec:2_prelim:mas_and_vec}), emphasizing their potential benefits and integration challenges.


\section{Edge Computing (EC)} \label{sec:2_prelim:edge_computing}

\glsreset{ec}



\subsection{Introduction to Edge Computing} \label{sec:2_prelim:ec_intro}

\gls{ec} extends cloud computing services closer to the end user, addressing high latency and mobility challenges inherent in traditional cloud models. By positioning computational resources at the network's edge, \gls{ec} enhances application responsiveness and real-time data processing by improving speed and efficiency. This is particularly beneficial with the \gls{ioe}, where the proliferation of smart devices generates vast amounts of data that require efficient local processing.~\cite{Cao2020, Khan2019}

Key characteristics of \gls{ec} include dense geographical distribution, mobility support, location awareness, and proximity to users, contributing to low latency and context awareness.~\cite{Khan2019} 
Local data processing at the edge enhances security, reduces bandwidth usage, and improves energy efficiency.~\cite{Cao2020} 

\gls{ec} architecture typically involves four layers: the device layer, the edge layer, the fog layer, and the cloud layer. The device (or terminal) layer includes all connected devices, while the edge layer consists of nodes like base stations and edge servers that provide localized processing. The fog layer acts as an intermediary, extending the capabilities of the edge by providing additional computational resources and storage and enabling more complex processing closer to the data source. The cloud layer handles large-scale data analysis and long-term storage, providing global insights and centralized management~\cite{Cao2020, Khan2019}.

Security and privacy are crucial in \gls{ec}, involving encryption, secure data sharing, identity authentication, and privacy protection measures. The ability to employ fine-grained access control further enhances security.~\cite{Cao2020} 

\gls{ec} applications include video caching, 5G communication, network video live broadcasting, predictive maintenance, and security monitoring. Integration with 5G networks leverages \gls{ec} for faster processing and low latency, enhancing these networks' capabilities.~\cite{Cao2020, Khan2019}



\subsection{General Network Setup} \label{sec:2_prelim_network_setup}

In \gls{ec}, the network setup strategically deploys computational resources and networking capabilities to improve performance, security, and scalability. This setup is crucial for ensuring efficient data processing, low latency, and an enhanced user experience, particularly in situations that demand quick response times and localized data handling.~\cite{Alkaabi2024, Cao2020, Khan2019} 

\subsubsection{Key Components}

\begin{itemize}
\item \textbf{Base Stations}: Base stations are essential components of \gls{ec} architectures, serving as the primary contact points for end-user devices and managing local data processing and transmission. In mobile networks, these stations are equipped with computational capabilities, traditionally found in centralized cloud servers, which help to decrease latency and enhance application responsiveness.~\cite{Alkaabi2024, Cao2020, Khan2019}

\item \textbf{Edge Servers}: Distributed across numerous locations, edge servers are strategically positioned closer to end-users than traditional cloud data centers. They manage data storage, processing, and real-time analytics, effectively minimizing the data transmitted to the cloud, thereby lowering latency and bandwidth usage. These servers can be in cellular base stations, Wi-Fi routers, or dedicated edge data centers.~\cite{Cao2020, Khan2019}

\item \textbf{Gateways}: Gateways serve as intermediaries between end-user devices and edge servers. They aggregate data from multiple sources, perform initial data filtering and preprocessing, and then forward relevant information for further processing. Gateways are essential for managing data traffic and ensuring efficient communication within the network.~\cite{Alkaabi2024, Cao2020, Khan2019}

\item \textbf{Access Points (APs)}: Wi-Fi routers and similar devices function as access points, enabling connectivity for end-user devices and linking local networks with the wider \gls{ec} infrastructure. Additionally, they can process and cache data to improve performance and minimize latency.~\cite{Khan2019}

\end{itemize}

\subsubsection{Deployment Strategies}

\begin{itemize}
\item \textbf{Proximity-Based Deployment:} The deployment of edge servers and base stations near end-users has been shown to minimize latency and enhance data processing speeds. This particularly benefits urban areas with high data traffic and user density.~\cite{Khan2019}

\item \textbf{Regional Data Centers:} The establishment of regional data centers with edge servers facilitates geographically distributed data processing, effectively balancing the load across the network and reducing reliance on centralized cloud data centers.~\cite{Khan2019}

\item \textbf{Hybrid Deployment:} A hybrid deployment model that integrates edge and cloud resources allows for flexible data processing and storage. Mission-critical and latency-sensitive applications can be handled at the edge, while less time-sensitive tasks can be processed in the cloud.~\cite{Khan2019}

\end{itemize}



\section{Multi-Access Edge Computing (MEC)} \label{sec:2_prelim:ec:mec}

\glsreset{mec}
\gls{mec}, or Mobile Edge Computing, is a specialized form of \gls{ec} tailored for mobile environments and specifically addresses the unique challenges of mobile networks, such as high mobility and frequent handovers.~\cite{Mach2017}

\subsection{Distinction Between General \gls{ec} and \gls{mec}}

While general \gls{ec} reduces latency and improves bandwidth efficiency by processing data near its source, \gls{mec} extends these benefits to highly mobile scenarios by integrating cloud capabilities within the network's edge infrastructure. This integration allows for low-latency, high-bandwidth services to be delivered directly from base stations and other edge nodes, which is critical for applications requiring rapid data processing and minimal latency, such as \gls{ar}, \gls{vr}, and \gls{ad}.~\cite{Mach2017, Mao2017}

A key distinction of \gls{mec} is its inherent support for mobility. Mobile devices frequently change their point of attachment to the network, necessitating robust handover mechanisms that ensure service continuity without performance degradation. This involves maintaining network connectivity and guaranteeing the seamless transfer of application states and data between edge nodes.~\cite{Alkaabi2024}


\subsection{Traditional Handover in Cellular Networks} \label{sec:2_prelim:traditional_handover}

Handover is a fundamental mechanism in cellular networks, facilitating the transfer of an ongoing call or data session from one cell to another as a user moves through the network. This process is critical for maintaining service continuity and quality. Traditional handover mechanisms rely on several triggers and methods to optimize performance and reduce disruptions.~\cite{Pollini1996}

The most straightforward method uses the \gls{rss} of the current and candidate base stations. The handover occurs when the signal from the new base station becomes stronger than the current one, although this can lead to frequent and unnecessary handovers if the current signal is still adequate. To improve this, methods such as \gls{rss} with thresholds and hysteresis are employed. Thresholds ensure that the current signal must drop below a certain level before a handover is initiated, while hysteresis margins prevent the ping-pong effect, where a mobile repeatedly switches between two cells. Advanced techniques also include prediction-based methods, which forecast future signal strength to initiate handovers before the signal deteriorates significantly.~\cite{Pollini1996}

Timers, such as dwell timers, are introduced to manage handover frequency, ensuring that a mobile device must stay connected to a new base station for a minimum period before another handover can occur. Dynamically adjusting hysteresis margins based on network conditions can further reduce unnecessary handovers and improve overall system performance.~\cite{Pollini1996}

\subsubsection{Handover Performance Metrics}

Performance metrics for handover include call blocking probability, handover blocking probability, handover probability, call dropping probability, rate of handover, duration of interruption, and delay. These metrics are essential for evaluating the efficiency and reliability of handover processes in cellular networks.~\cite{Pollini1996}

\subsubsection{Soft vs Hard Handover}

\glsreset{hho}
\glsreset{sho}

In terms of handover types, \gls{hho} involves breaking the old connection before the new one is activated, leading to brief service interruptions. In contrast, \gls{sho} establishes the new connection before releasing the old one, providing a seamless transition with no service interruption.~\cite{Pollini1996}

In summary, understanding traditional handover mechanisms and their triggers is crucial for developing advanced handover strategies in \gls{mec}. These conventional methods lay the groundwork for more sophisticated approaches needed to handle the high mobility and low latency requirements of modern networks.~\cite{Pollini1996}



\subsection{Challenges and Solutions} \label{sec:2_prelim:challenges_solutions}

Managing the handover process is a core challenge in \gls{mec}. Mobile devices move between different network cells, requiring a seamless transition of active sessions and services from one \gls{mec} server to another. This handover process must be efficient to avoid service interruptions and maintain \gls{qos}.~\cite{Mao2017}


\subsubsection{Imperative vs. Alternative Handovers} \label{sec:2_prelim:imp_alt_ho}

Imperative handovers are critical for maintaining system stability and \gls{qos}. They are executed to prevent the mobile device from losing connectivity (when leaving the \gls{mec} station's range) or to avoid the \gls{mec} station from being overloaded. In contrast, alternative handovers are not strictly necessary but can enhance system performance by balancing loads more effectively across \glspl{mec} station. These handovers are initiated based on the potential to improve overall system efficiency and resource utilization.


\subsubsection{Handover Strategies}

\begin{enumerate}
\item \textbf{Handover Protocols}: \gls{mec} utilizes specialized handover protocols that differ from traditional mobile handovers. These protocols ensure that not just the network connection but also the application state and user context are smoothly transferred.~\cite{Alkaabi2024, Li2016}

\item \textbf{Stateful and Stateless Migration}: \gls{mec} supports both stateful and stateless migration of services. Stateful migration involves transferring the entire application state, including memory and processing status, to the new \gls{mec} node. This allows the new node to resume precisely where the old one left off, thereby providing a seamless user experience. Stateless migration moves only the computation tasks, with session states reconstructed at the new node.~\cite{Mao2017, Alkaabi2024}

\item \textbf{Virtual Machine and Container Migration}: Techniques such as \gls{vm} and container migration are employed to move application instances between \gls{mec} nodes. Live migration techniques minimize downtime and service disruption.~\cite{Mao2017, Alkaabi2024}

\end{enumerate}

\subsubsection{Resource Allocation and Management}

Effective resource management is crucial in \gls{mec}. Nodes must dynamically allocate resources to handle varying workloads while ensuring optimal performance and low latency:

\begin{enumerate}
\item \textbf{Dynamic Resource Allocation}: Algorithms for dynamic resource allocation help \gls{mec} nodes efficiently manage computing, storage, and network resources. These algorithms consider factors such as current load, predicted future demand, and \gls{qos} requirements to make real-time decisions.~\cite{Alkaabi2024, Mach2017, Mao2017}

\item \textbf{Load Balancing}: Effective load balancing strategies are crucial to prevent any single \gls{mec} node from becoming a bottleneck. This involves distributing the workload evenly across multiple nodes to ensure high availability and reliability.~\cite{Alkaabi2024, Mao2017}

\end{enumerate}

\subsection{Specific Techniques and Processes}

\subsubsection{Handover Processes}

The handover process in \gls{mec} involves several steps to ensure a seamless service transition:

\begin{enumerate}
\item \textbf{Network Discovery}: Before initiating a handover, the \gls{mec} system performs network discovery to identify potential target nodes that can accommodate the migrating service.~\cite{Alkaabi2024}

\item \textbf{Decision Phase}: Once potential targets are identified, the system decides the optimal target based on criteria such as current load, latency, and resource availability.~\cite{Alkaabi2024, Mao2017}

\item \textbf{Execution Phase}: The actual handover involves migrating the application state, re-routing the network traffic, and updating the user context at the new \gls{mec} node. Techniques such as live migration ensure that this process happens with minimal disruption.~\cite{Alkaabi2024, Mao2017}

\end{enumerate}

\subsection{Handover in LTE vs. MEC}

In traditional cellular networks like LTE networks, handover procedures are critical for maintaining ongoing connections and ensuring service continuity, as described in Section~\ref{sec:2_prelim:traditional_handover}. The handover process in LTE typically involves three phases: preparation, execution, and completion:~\cite{Li2016}


\begin{enumerate}
\item \textbf{Preparation Phase}: This phase involves the source LTE node selecting a target node based on measurement reports from the \gls{ue}. The source node sends a handover request to the target node, which then performs admission control and allocates resources for the \gls{ue}.~\cite{Li2016}

\item \textbf{Execution Phase}: The \gls{ue} disconnects from the source node and connects to the target node. Once connected, the \gls{ue} sends a handover confirmation message to the target node to start receiving data.~\cite{Li2016}

\item \textbf{Completion Phase}: This phase involves switching the downlink path to inform the core network entities to switch the data path from the source node to the target node and release the resources allocated to the \gls{ue} in the source cell.~\cite{Li2016}

\end{enumerate}




In summary, \gls{mec} distinguishes itself from general \gls{ec} through its robust support for mobility and seamless handover processes. By addressing the challenges of mobile environments, \gls{mec} enables a wide range of applications requiring low latency and high reliability, such as \gls{ad} and real-time video analytics. Effective resource management and advanced migration techniques ensure these services remain uninterrupted as devices move across the network.



\section{Vehicular Edge Computing (VEC)} \label{sec:2_prelim:ec:vec}

\glsreset{vec}
\gls{vec} is a specialized form of \gls{ec} that integrates \gls{mec} capabilities within vehicular networks. By design, \gls{vec} addresses the high mobility, real-time data processing needs, and significant computational requirements of modern vehicular applications, such as \gls{ad}, \gls{ar}, \gls{vr}, and online gaming.~\cite{Huang2020, Liu2021}


\subsection{Key characteristics and components of VEC}

\gls{vec} systems are characterized by their ability to handle dynamic and highly mobile environments. The key components of \gls{vec} include the \gls{rsu}, the vehicular \gls{obu}, and \gls{mec} servers.

\textbf{RSUs and OBUs}: \gls{rsu}s are deployed along the roads and serve as the primary communication points for vehicles. They facilitate \gls{v2i} communication. \gls{obu}s, installed in vehicles, handle data collection and preliminary processing.~\cite{Huang2020, Liu2021}

\textbf{MEC Servers}: These servers are typically colocated with \gls{rsu}s and provide significant computational resources for processing tasks offloaded from vehicles. This colocation minimizes the distance data needs to travel, thereby reducing latency and energy consumption.~\cite{Huang2020, Liu2021}


\subsection{Benefits of VEC}

The integration of \gls{ec} into vehicular networks offers multiple benefits:
\begin{itemize}
\item \textbf{Reduced Latency}: By processing data at the edge of the network, \gls{vec} significantly reduces the time required for data transmission, making it ideal for real-time applications.~\cite{Huang2020, Liu2021}
\item \textbf{Energy Efficiency}: Offloading computation-intensive tasks to nearby \gls{mec} servers reduces the energy consumption of vehicular \gls{obu}s, thereby extending the operational time of these units.~\cite{Huang2020, Liu2021}
\item \textbf{Enhanced Data Processing}: \gls{vec} systems can handle large volumes of data generated by vehicular sensors and applications, providing faster and more reliable data processing.~\cite{Huang2020, Liu2021}
\end{itemize}


\subsection{Challenges in VEC}

Despite its benefits, VEC faces several challenges:
\begin{itemize}
\item \textbf{Mobility Management:} High mobility, characterized by the rapid and continuous movement of vehicles, necessitates robust handover mechanisms to maintain stable connectivity between \glspl{rsu} and \gls{mec} servers.~\cite{Huang2020, Liu2021}
\item \textbf{Task Offloading Decisions:} Making optimal offloading decisions is crucial for minimizing energy consumption and ensuring low packet drop rates. Dynamic task offloading schemes are essential for adapting to varying network conditions and vehicle mobility.~\cite{Huang2020, Liu2021}
\item \textbf{Resource Allocation:} Efficient allocation of computational resources among multiple vehicles is necessary to avoid congestion and ensure high \gls{qos}. Algorithms for dynamic resource allocation help manage the varying workloads and maintain system stability.~\cite{Huang2020, Liu2021}
\end{itemize}


\subsection{VEC in practice}

In practical implementations, \gls{vec} systems use a combination of communication technologies such as \gls{dsrc}, Wi-Fi, and cellular networks for \gls{v2i} communication. \gls{mec} servers colocated with \gls{rsu}s handle the offloaded tasks from vehicles, providing a powerful infrastructure for computation-intensive applications while reducing execution time and local energy consumption.~\cite{Huang2020, Liu2021}

The deployment strategies in \gls{vec} involve placing \gls{mec} servers and \gls{rsu}s in strategic locations to ensure optimal coverage and minimal latency. This setup is particularly beneficial in urban areas with dense traffic, with high demand for real-time data processing.~\cite{Huang2020, Liu2021}




As shown in Table \ref{tab:2_prelim:ec_mec_vec_comparison}, there are key distinctions between \gls{ec}, \gls{mec}, and \gls{vec} in terms of focus, mobility, key applications, infrastructure, and challenges.

\begin{table}
\centering
\caption{Differentiation of \gls{ec}, \gls{mec}, and \gls{vec}}
\label{tab:2_prelim:ec_mec_vec_comparison}
\begin{tabularx}{\textwidth}{|l|X|X|X|}
\hline
\textbf{Feature}        & \textbf{\gls{ec}}                       & \textbf{\gls{mec}}              & \textbf{\gls{vec}}                \\ \hline
\textbf{Focus}          & General edge processing near the end-user.          & \gls{ec} tailored for mobile networks.            & \gls{ec} specialized for vehicular networks.     \\ \hline
\textbf{Mobility}       & Limited mobility support.                           & High mobility support with seamless handovers.          & Very high mobility with rapid \gls{v2i} handovers. \\ \hline
\textbf{Key Applications} & \gls{iot}, smart cities, local data processing.          & Mobile services, \gls{ar}/\gls{vr}, low-latency mobile applications. & \gls{ad}, \gls{v2x} communication, real-time vehicle data processing. \\ \hline
\textbf{Infrastructure} & Edge servers, gateways, and \glspl{ap}.          & Edge servers integrated with mobile base stations.      & \glspl{rsu}, \glspl{obu}, \gls{mec} servers. \\ \hline
\textbf{Challenges}     & Resource management, security, latency reduction.   & Seamless mobility, dynamic resource allocation.         & High mobility management, low-latency processing under vehicular dynamics. \\ \hline
\end{tabularx}
\end{table}




\section{Multi-Agent Systems (MAS)} \label{sec:2_prelim:mas}

\glsreset{mas}
\glspl{mas} are a subset of \gls{dai} where multiple agents interact within a common environment to achieve specific goals. These systems have gained traction due to their ability to handle complex, distributed, and dynamic problems more efficiently than traditional systems. The fundamental concept involves agents working collaboratively or competitively to solve problems beyond the capabilities of individual agents.~\cite{Balaji2010, McArthur2007_1}

This structured overview provides a foundational understanding of \glspl{mas}, setting the stage for exploring their integration into \gls{vec} for task handover coordination. The detailed examination of agents, communication, and coordination strategies will be critical for developing effective \gls{mas} solutions in this domain.

\subsection{Agents in \glspl{mas}}

Balaji et al.~\cite{Balaji2010} define an agent in \glspl{mas} as a flexible, autonomous entity capable of perceiving its environment through sensors and acting upon it using actuators. According to them, agents possess several key properties:
\begin{itemize}
\item \textbf{Situatedness}: Interaction with the environment, encompassing both input and output, is direct and integral to the agent’s design.
\item \textbf{Autonomy}: Agents operate independently without external intervention, thereby isolating them from instability. 
\item \textbf{Inferential capability}: Agents can deduce new information from available data, enabling them to achieve abstract and complex objectives.
\item \textbf{Responsiveness}: Agents can quickly adapt to changes in their environment.
\item \textbf{Proactiveness}: Agents not only respond to changes but also take initiative to achieve their goals.
\item \textbf{Social behavior}: Agents can communicate, collaborate, and share knowledge with other agents to accomplish tasks.
\end{itemize}


\subsection{Characteristics of \glspl{mas}}

\glsreset{mas}
A \gls{mas} extends agent technology by incorporating a collection of loosely interconnected autonomous agents operating within an environment to pursue a shared objective. These agents may cooperate or compete, and they may choose to share or withhold knowledge from one another.~\cite{Balaji2010, Sauvage2004}

These systems are characterized by \textbf{decentralization}, meaning there is no central control, which enhances robustness and scalability. \textbf{Parallelism} is another key characteristic where agents operate concurrently, boosting system performance. Additionally, \glspl{mas} exhibit \textbf{flexibility and adaptability}, dynamically adjusting to new tasks and environments.~\cite{Balaji2010, Sauvage2004}

\subsection{Challenges of \glspl{mas}}

Despite their advantages, \glspl{mas} face several challenges. 
\textbf{Coordination complexity} is a primary issue, as ensuring effective coordination among agents to prevent conflicts and inefficiencies can be difficult.
\textbf{Communication overhead} is another challenge involving the management of the volume of inter-agent communication to avoid performance bottlenecks.
\textbf{Scalability issues} arise as the number of agents increases, and maintaining system performance under these conditions can be challenging.
Moreover, \textbf{robustness and fault tolerance} are critical; \glspl{mas} must be designed to handle agent failures gracefully without affecting overall system performance.~\cite{Balaji2010, Sauvage2004, McArthur2007_1}


\subsection{Classifications of \glspl{mas}}

\glspl{mas} can be classified based on their organizational structure:

\begin{itemize}
\item \textbf{Hierarchical Organization}: Agents are organized in a hierarchy with clear roles and responsibilities.~\cite{Balaji2010}
\item \textbf{Flat Organization}: All agents have equal roles and responsibilities.~\cite{Balaji2010}
\item \textbf{Hybrid Organization}: Combines elements of both hierarchical and flat structures to leverage their advantages.~\cite{Balaji2010}
\end{itemize}

In addition, we also differentiate between homogeneous and heterogeneous structures.
In \textbf{homogeneous structures}, agents share identical internal setups (goals, sensors, states, inference mechanisms, and actions) and differ only in their physical location and the environment they interact with. This uniformity is typically seen in distributed environments, where sensor input overlap is rare.
Conversely, \textbf{heterogeneous structures} consist of agents with different abilities, structures, and functions, acting based on their specific environment and location. This diversity makes them more realistic and may result in conflicting goals.~\cite{Balaji2010}


\subsection{Performance metrics of \glspl{mas}}

Performance in \glspl{mas} can be evaluated using metrics such as response time, communication efficiency, and system robustness. These metrics help assess how well the \gls{mas} achieves its goals under various conditions. For example, response time is a critical metric in assessing the \gls{qos} in \glspl{mas}, particularly in systems with intensive communications like crisis management and cinema ticket selling scenarios.~\cite{Balaji2010, Gutierrez2011}


\subsection{Decision-making in \glspl{mas}}

Agents in \glspl{mas} use various decision-making strategies to determine their actions. These strategies include:

\begin{itemize}
\item \textbf{Reactive Decision-Making}: Agents respond to changes in their environment in real-time.~\cite{Balaji2010}
\item \textbf{Deliberative Decision-Making}: Agents plan their actions based on predictions about the future state of the environment.~\cite{Balaji2010}
\item \textbf{Hybrid Decision-Making}: Combines reactive and deliberative approaches to balance immediate responses and long-term planning.~\cite{Balaji2010}
\end{itemize}

\subsection{Coordination in \glspl{mas}}

\begin{itemize}
\item \textbf{Protocols}: Sets of rules that define interactions between agents, such as the Contract Net Protocol, which manages task allocation among agents.~\cite{Sauvage2004}
\item \textbf{Organizational Structures}: Defines roles and relationships between agents, ensuring structured and efficient interactions.~\cite{Balaji2010}
\item \textbf{Negotiation and Auctions}: Agents negotiate or bid for tasks to optimize resource allocation and task distribution.~\cite{Balaji2010, Sauvage2004}
\end{itemize}




\subsection{Communication Patterns for \glspl{mas}} \label{sec:2_prelim:comm_patterns}

Communication patterns ensure efficient and reliable data exchange among interconnected devices and systems within \glspl{mas}. These patterns, which include request-response, publish-subscribe, discovery, message passing, and blackboard, provide solutions tailored to the unique requirements of \glspl{mas}, allowing for better system interaction and coordination.~\cite{Carlier2020, Eugster2003, Henneke2015}


\subsubsection{Request-Response}

In \glspl{mas}, the request-response pattern is used for direct interactions where one agent (requester) sends a request to another agent (responder) and awaits a response. This pattern is often employed in task delegation and service provision among agents. Unlike traditional systems, \gls{mas} agents can dynamically switch roles between requester and responder, enhancing flexibility. However, the challenge lies in managing these dynamic roles and ensuring timely responses to maintain overall system performance. The pattern is handy for scenarios requiring immediate and deterministic responses but may introduce bottlenecks if many agents simultaneously request responses from a single agent.~\cite{Carlier2020, Eugster2003, Henneke2015, Siedler2021}

\subsubsection{Publish-Subscribe}

The publish-subscribe pattern in \glspl{mas} supports asynchronous communication, where agents publish messages to specific topics, and other agents subscribe to these topics to receive updates. This decoupling allows for flexible and scalable communication, making it effective in large-scale \glspl{mas}. Agents use the publish-subscribe pattern to disseminate information about environmental changes, state updates, or resource availability. Acting as a neutral mediator, the event service propagates events to all relevant subscribers without needing publishers and subscribers to know each other. This decoupling in space, time, and synchronization makes the pattern highly flexible and scalable.~\cite{Carlier2020, Eugster2003, Mataric1998}

\subsubsection{Discovery}

Discovery patterns enable agents to locate and connect dynamically without prior knowledge of network addresses. This capability is essential in environments where agents frequently join or leave the system. \glspl{mas} often implement sophisticated discovery algorithms that allow agents to identify potential collaborators or competitors based on their goals and current states. Discovery services support dynamic, real-time interactions and adapt to the constantly changing agent configurations, enhancing the system's adaptability and responsiveness.~\cite{Carlier2020, Henneke2015, Siedler2021}

\subsubsection{Message Passing}

Message passing in \glspl{mas} is vital for direct agent-to-agent communication, supporting synchronous and asynchronous interactions. This pattern ensures real-time coordination and cooperation among agents. Optimized message-passing protocols handle high volumes of messages efficiently, maintaining low latency and reliability. Agents use this method to share state information, coordinate actions, and negotiate resources. Effective message-passing designs prevent communication bottlenecks and prioritize critical messages for timely delivery, ensuring the smooth operation of the \gls{mas}.~\cite{Balaji2010, Siedler2021} 
Fault tolerance and reliability can be enhanced by incorporating redundancy in communication paths and error correction techniques, ensuring robust message delivery despite failures.~\cite{Gutierrez2011}

\subsubsection{Blackboard}

The blackboard pattern in \glspl{mas} acts as a shared knowledge repository where agents post and retrieve information. This pattern is particularly effective for collaborative problem-solving, requiring collective intelligence and coordination among multiple agents. Enhanced blackboard systems handle concurrency and prioritize critical information, allowing agents to share partial solutions, update task statuses, and coordinate activities, without direct communication. This indirect communication method simplifies managing complexity and ensures all agents access the latest necessary information for decision-making.~\cite{Carlier2020, Sauvage2004} 
Advanced techniques, such as \gls{ml}, can optimize the blackboard's efficiency, predicting which information will be needed and preemptively organizing it.~\cite{Balaji2010}


==> sections/experimental_setup/subsec_RSAgent_parameters.tex <==
\subsection{\gls{rs} Agent Strategy Parametrization} \label{sec:6_eval:rs_agent_parametrization}

This section focuses on determining the optimal strategy constants for the \gls{rs} agents through a series of experiments. All experiments were performed with the highest possible load-sharing frequency, set to 1, meaning load information is shared after each timestep.

\subsubsection{Scenario for Parameter Tuning}

The experiments utilized the Créteil morning scenario with a 4 \gls{rsu} setup, each operating at halved capacity, as described in Section~\ref{sec:6_eval:creteil_rsu_config_sparse}. This configuration was selected due to its challenging environment, characterized by high traffic density and limited \gls{rsu} capacity, making it an effective stress test for the strategies. By pushing the system toward its operational limits, we can identify parameters that ensure robust performance even under less favorable conditions.

This sparse setup forces the \gls{rs} agents to make critical handover and load-balancing decisions, essential for identifying optimal strategy parameters. It represents the most demanding scenario the \gls{rs} agents might encounter, ensuring that the selected parameters will be effective across various configurations.

Once optimized under these challenging conditions, these parameters were applied to all subsequent experiments, including those with the denser configuration of nine \glspl{rsu}. This approach ensures that the parameters are effective in high-stress scenarios and adaptable to varying network densities, guaranteeing consistent \gls{qos} and efficient load balancing in all configurations.



The following parameters for the proposed strategy, detailed in Section~\ref{sec:5_impl:rs_agent_impl}, were tuned:
\begin{itemize}
\item \textbf{Leaving Threshold}: Percentage of the \gls{rsu}'s range at which the \gls{rsu} will hand over the vehicle if it is outside the inner part of the range. For example, if the threshold is 90\% and the range is 50 meters, the vehicle will be handed over if it is more than 45 meters away from the \gls{rsu}.
\item \textbf{Overload Threshold}: Percentage of the \gls{rsu}'s capacity at which handovers of the most suitable vehicles will be forced when the load percentage exceeds this threshold.
\item \textbf{Load-Balancing Hysteresis}: Margin for utilization percentage difference that another \gls{rsu} must be lower than the current one to justify a handover. This margin is applied to either an alternative handover to a less utilized \gls{rsu} or an imperative handover if the current \gls{rsu} is overloaded. The load of the considered vehicle is added to the other \gls{rsu}'s load before comparison.
\item \textbf{Load-Balancing Minimum Suitability}: Minimum suitability another station should have for a vehicle to be considered for a handover, based on the suitability score presented in Section~\ref{sec:5_impl:rs_heuristics}. This is ignored if the source \gls{rsu} is overloaded.
\end{itemize}



\subsubsection{General Observations}

\begin{enumerate}
\item \textbf{Leaving Threshold}: Reducing the leaving threshold improves all metrics, with setting the leaving range to 0 yields the best results across the board, replicating the latest \gls{ho} strategy for mobility-caused handovers.
\item \textbf{Overload-triggered Handover}: Overload-triggered handovers are infrequently used, as load-balancing effectively addresses these situations in nearly all evaluated strategy configurations.
\item \textbf{Handover Frequency}: Minimizing the number of handovers requires a combination of high load-balancing hysteresis, high minimum suitability, and a high overload threshold.
\item \textbf{Maximizing \gls{qos}}: Both average and minimum \gls{qos} are maximized with minimal load-balancing hysteresis.
\item \textbf{Minimizing Gini Coefficient}: Achieving a low Gini coefficient requires minimal load-balancing hysteresis, overload threshold, and suitability.
\item \textbf{Visualization}: Visual analysis of specific configurations revealed the causes of unexpected behaviors and aided in identifying implementation bugs.
\end{enumerate}



\subsubsection{Finding the Best Parameters}

Identifying the best parameters in this search space was challenging. Two evaluation metrics were introduced, relevant only to the parameter selection:

\begin{itemize}
\item \textbf{Normalization Process}

\begin{itemize}
\item Each criterion's score is normalized to a value between 0 and 1.
\item For handover count and Gini coefficient, where lower values are better, the normalization formula used is:
$$ \text{Normalized Score} = \frac{\text{Minimum Observed Value}}{\text{Observed Value}} $$
\item For average \gls{qos} and minimum \gls{qos}, where higher values are better, the normalization formula used is:
$$ \text{Normalized Score} = \frac{\text{Observed Value}}{\text{Maximum Observed Value}} $$
\item This normalization ensures that the best possible score for each criterion is 1, and lower scores reflect worse performance relative to the best-observed performance.
\end{itemize}



\item \textbf{Evaluation Scores}
\begin{itemize}
\item \textbf{Evaluation Sum}: The sum of normalized scores for handover count, average \gls{qos}, minimum \gls{qos}, and Gini coefficient.
\item \textbf{Evaluation Product}: The product of the same normalized scores, which is more sensitive to outliers.
\end{itemize}
\end{itemize}

The normalized scores range between 0 and 1, with 1 representing the best possible score. The top parameter configurations, as determined by both metrics, are shown in Table~\ref{tab:6_eval:rs_strat_top_params}.


\begin{table}
\centering
\caption{Top \gls{rs} Agent Strategy Parameter Configurations}
\label{tab:6_eval:rs_strat_top_params}
\begin{tabular}{|c|c|c|r|r|}
\hline
\textbf{Overload} & \textbf{Hysteresis} & \textbf{Suitability} & \textbf{Eval Sum} & \textbf{Eval Product} \\
\hline
0.7 & 0.05 & 0.3  & 3.8175 & 0.8252 \\
0.6 & 0.05 & 0.35 & 3.8159 & 0.8236 \\
0.8 & 0.05 & 0.25 & 3.8151 & 0.8232 \\
0.9 & 0.05 & 0.2  & 3.8137 & 0.8216 \\
0.8 & 0.05 & 0.2  & 3.8137 & 0.8215 \\
\hline
\end{tabular}
\end{table}

These results indicate that a load-balancing hysteresis of 0.05 is the most effective strategy. The optimal overload threshold is 0.7, while a load-balancing minimum suitability of 0.3 emerges as the top choice, closely aligning with the average of the highest-performing values. This combination provides a balanced and efficient approach for managing handovers and maintaining \gls{qos} in the tested scenarios.




\subsubsection{Chosen Parameters for \gls{rs} Agent Strategy}
Based on the analysis, the following \gls{rs} agent strategy parameters were selected for all subsequent experiments:

\begin{itemize}
\item \textbf{Leaving Threshold}: 0
\item \textbf{Overload Threshold}: 0.7
\item \textbf{Load-Balancing Hysteresis}: 0.05
\item \textbf{Load-Balancing Minimum Suitability}: 0.3

\end{itemize}


These parameters will be used to evaluate the performance of the \gls{rs} agent strategies in subsequent experiments, ensuring a balance between minimizing handovers, maximizing \gls{qos}, and maintaining fairness in load distribution.







